Homologies of path complexes and digraphs

In this paper we introduce a path complex that can be regarded as a generalization of the notion of a simplicial complex. The main motivation for considering path complexes comes from directed graphs(digraphs). We obtain a new notion of the path homology and cohomology of a digraph.

==> tcidefs.tex <==

\def\BibDimMuGauge{1}
\def\BibGrigMuralg{2}
\def\BibGrigMurYauhh{3}
\def\BibHiltonWylie{4}
\def\BibMacLane{5}
\def\BibAli{6}
